High-resolution transmission spectroscopy of the hot-Saturn HD 149026b

Advances in modern technologies enable the characterisation of exoplanetary atmospheres, most efficiently exploiting the transmission spectroscopy technique. We performed visible (VIS) and near infrared (nIR) high-resolution spectroscopic observations of one transit of HD 149026b, a close-in orbit sub Saturn exoplanet. We first analysed the radial velocity data, refining the value of the projected spin-orbit obliquity. Then we performed transmission spectroscopy, looking for absorption signals from the planetary atmosphere. We find no evidence for H$\alpha$, NaI D2 - D1, MgI and LiI in the VIS and metastable helium triplet HeI(2$^3$S) in the nIR using a line-by-line approach. The non-detection of HeI is also supported by theoretical simulations. With the use of the cross-correlation technique, we do not detect TiI, VI, CrI, FeI and VO in the visible, and CH$_4$, CO$_2$, H$_2$O, HCN, NH$_3$, VO in the nIR. Our non-detection of TiI in the planetary atmosphere is in contrast with a previous detection. We performed injection-retrieval tests, finding that our dataset is sensitive to our TiI model. The non-detection supports the TiI cold-trap theory, which is valid for planets with $T_{\rm eq} <$ 2200 K like HD 149026b. Even if we do not attribute it directly to the planet, we find a possibly significant TiI signal highly redshifted ($\simeq$+20 km s$^{-1}$) with respect to the planetary restframe. Redshifted signals are also found in the FeI and CrI maps. While we can exclude an eccentric orbit to cause it, we investigated the possibility of material accretion falling onto the star, possibly supported by the presence of strong LiI in the stellar spectrum, without finding conclusive results. The analysis of multiple transits datasets could shed more light on this target.

==> Tabelle/tabella_posterior.tex <==
\begin{table}
\centering
\renewcommand{\arraystretch}{1.0}
\fontsize{7}{13}\selectfont
\caption{Posterior distributions from the MCMC.}
\label{table:4}
\begin{tabular}{
m{2.5cm}
P{2.5cm}
}
\hline
\hline
% -------------------------
Parameter &
Posterior Values [Unit]\\
% -------------------------
\hline
$V_{sys}$  &
     \,\, [km/s] \\

$R_p/R_{*}$ &
    \\

$v \sin{i}$ &
     \,\, [km/s] \\

$K$ &
     \,\, [km/s] \\

$\log{\sigma_w}$ &
    \\

$i$ &
     \,\, [deg] \\

$\lambda$ &
     \,\, [deg] \\

$\delta T_0$ &
     \,\, [Phase] \\
\hline
\hline
\end{tabular}
\end{table}
